OCCAM: An Optimization-Based Approach to Network Inference

We study the problem of inferring the structure of a communication network based only on network measurements made from a set of hosts situated at the network periphery. Our novel approach called "OCCAM" is based on the principle of occam's razor and finds the "simplest" network that explains the observed network measurements. OCCAM infers the internal topology of a communication network, including the internal nodes and links of the network that are not amenable to direct measurement. In addition to network topology, OCCAM infers the routing paths that packets take between the hosts. OCCAM uses path metrics measurable from the hosts and expresses the observed measurements as constraints of a mixed-integer bilinear optimization problem that can then be feasibly solved to yield the network topology and the routing paths. We empirically validate OCCAM on a wide variety of real-world ISP networks and show that its inferences agree closely with the ground truth. Specifically, OCCAM infers the topology with an average network similarity score of 93% and infers routing paths with a path edit distance of 0.20. Further, OCCAM is robust to error in its measured path metric inputs, producing high quality inferences even when 20-30% of its inputs are erroneous. Our work is a significant advance in network tomography as it proposes and empirically evaluates the first method that infers the complete network topology, rather than just logical routing trees from sources.

==> related.tex <==
\section{Related Work}
\label{sec:related}

Inferring the network topology and routing paths from end-to-end measurements  is an important  area with more than two decades of research. One thrust has explored the use of active probes (such as  traceroute and mtrace) and data feeds  (such as BGP) to infer the network topology and routes.  For example, Skitter \cite{Claffy} and its successor Archipelago \cite{CAIDA2015} derives the router-level and AS-level topology of the Internet using traceroutes and BGP tables.  Rocketfuel \cite{Spring2004} infers the router-level topology of an ISP using traceroutes, BGP, and DNS measurements. \textcolor{blue}{Dimes \cite{Shavitt2005} aims to infer a fine grained router level topology by running traceroutes from application installed by volunteers on their personal computers, as opposed to previous methods that use dedicated machines. Doubletree \cite{Donnet2004} modifies traceroute to be more efficient by making the assumption that paths from a source or paths to a destination form a tree.}

%Active probing techniques require that routers in the network are cooperative, adhere to the Internet Congestion Message Protocol (ICMP) and respond to traceroute requests. However, %many routers in the network block traceroute requests due to security and privacy reasons \ref{} \ref{}. Thus, the traditional approaches detect the presence of such routers, but fail to %recover their identity. In the presence of such anonymous routers, \ref{} \ref{} tackle the problem of resolving anonymous routers to recover a minimal network topology consistent with %the probes. It is shown that the problem is NP-Complete and producing an approximate solution is intractable as well. The authors propose a couple of heuristics to solve the problem, %without any guarantees on the accuracy of the inference.  

Note that the above work require the network to support specific types of active probes (e.g, traceroutes) and/or to provide measurement feeds (e.g., BGP). However, for reasons of security, many networks (e.g., military networks) do not allow probes such as traceroutes and do not expose other internal network data that may be used for inference \cite{}.  Even in civilian networks such as the Internet, an increasing fraction of routers do not respond to  traceroutes \cite{Yao2003, Gunes2009}.  Further, future networks may obfuscate topology inference by returning false traceroute measurements \cite{TrassareEtAl}. Such considerations have led to research in ``network tomography'' that aim to infer  topology and routes with minimal co-operation from the network elements (i.e., no traceroutes or data feeds) \cite{vardi1996network,Castro2004,Bu2002,Duffield2002,presti2002multicast,caceres1999multicast}. Our work  provides the first empirically-validated technique for inferring the complete topology and routes in real-world networks under this setting.

We now place our work in the context of nearly two decades of network tomography research on topology and route inference. Early work focused on inferring the logical source tree rooted at host, not the entire network. Sylvia et al. \cite{Ratnasamy1999} propose a method to infer a logical binary source tree rooted at a source host with other receiver hosts as leaves. Multicast probes are sent from source host to a set of receivers. The tree is constructed on the observation that receivers experiencing correlated losses have a common shared path from the source, \textcolor{blue}{and the measure of correlation increases with the length of the shared path}. Subsequently, these results were extended to infer non-binary source trees with theoretical guarantees \cite{Duffield2002}.  Later, it was shown that source trees can be constructed using delay covariances measured at the hosts, instead of losses that may be rare on the Internet \cite{Duffield2004}. \textcolor{blue}{In \cite{Bowden2018}, it is shown that a tree topology can be inferred for networks in which link processes have non trivial spatial dependencies; previous techniques built on a strong assumption of mutual independence of link processes}. \textcolor{blue}{If multicast is not available, there is prior literature on using a train of unicast packets instead \cite{Duffield2006}.} 
\begin{comment}
 Our techniques for collecting PSM metrics using a train of unicast packets on DETER is directly derived from prior work above that uses such techniques to construct the source trees. It has also pointed out in prior literature measuring PSMs from unicast probes can be error-prone \cite{Duffield2006}, which was also our observation in our DETER experiments.
\end{comment}

While the above work infer single trees in isolation, there has been work on understanding how multiple source trees intersect  each other.  Given two source trees, \cite{Rabbat2004,Coates2003} shows how to discover the links where the trees intersect, using path sharing metrics between pairs of sources and destinations. However, the technique does not allow the trees to be merged into a single network, unless the trees overlap in very specific ways that do not hold for general topologies. Thus, these techniques cannot be used to produce the complete topology and routes as we do in our work.

Recently, there has been some work on complete topology and route inference. It is known that a sparse random graph with shortest-path routing can be inferred using \textcolor{red}{path sharing metrics} between pairs of sources and destinations, with small error and high probability \cite{Anandkumar2011}.  Concurrent to our work, that has been an interesting theoretical advance that shows that certain classes of graph topologies can be inferred using stronger primitives that allow the measurement of distances from hosts to certain internal nodes \cite{Berkolaiko2018}. Specifically, it is assumed that given paths from a host A to two hosts B and C, the individual distances from A, B, and C to the  internal node where the paths diverge can be measured. While it is not known how such a stronger primitive can be measured, our work uses only host-to-host distance measurements and also empirically validates the approach on real-world networks.



\begin{comment}
The goal of network tomography is to infer characteristics of the network, using passive measurements made from a subset of nodes, without relying on any cooperation from other nodes in the network.   The term \textit{network tomography} was first coined by Y. Vardi in \ref{}, in which the problem of estimating the traffic intensity between all source-destination pairs of nodes in the network using end to end probes was considered. In \ref{}, Sylvia et al. propose a method to infer a logical binary source tree rooted at a source host with other receiver hosts as leaves. Multicast probes are sent from source host to a set of receivers. The tree is constructed on the observation that receivers experiencing similar losses (correlated losses) have a common shared path from the source.\textcolor{red}{The algorithm iteratively finds a pair of nodes with maximum correlated losses, marks them as siblings and merges them into a single node. } Thus the algorithm returns a binary tree rooted at the source host with the other hosts as leaves. In \ref{}, extended the methodology and provided three algorithms to infer any generic logical tree along with theoretical guarantees.  The authors further extended the work to infer logical trees using delay correlation instead of loss correlation. The algorithm was made more efficient in \ref{}, for a special case of inferring a balanced n-ary tree. Building on techniques for inferring source trees Coates et al. addressed the problem of merging multiple source trees with the same set of receivers. Two source trees with the same set of receiver hosts (leaves) was mergeable, if and only if, the joining point of the path from the first source to a path from the second source can be localized to a single link in the source tree of the second host. This condition severely restricts the possible networks where the algorithm would infer the right network.  Also, the algorithm only infers DAGs.

To the best of our knowledge, there exists only a couple of algorithms \ref{} and \ref{} which claim to infer graphs using only passive measurements. The first algorithm assumes complete knowledge of all 2-by-2 components in the network. By a 2-by-2 component we mean the logical topology between any two source hosts and any two destination hosts along with the distances of each link in the logical topology. The algorithm also assumes the network is random graph which is locally tree-like. Under the given assumptions, the algorithm infers a graph with certain edit distance guarantees. The second algorithm \ref{} reconstructs the graph using the knowledge of 1-by-2 and 2-by-1 components in the network. The algorithm states the conditions under which the graph can be uniquely reconstructed. However, we believe that there exists no known techniques which can provide us with complete information of 2-by-2, 1-by-2 and 2-by-1 components of a network. Although the algorithms provide theoretical guarantees, both the algorithms do not work in practice.
\end{comment}

\begin{comment}
\textcolor{red}{
Our work falls within the broad area of network tomography \cite{vardi1996network,Castro2004} that seeks to infer metrics that are internal to the network using only measurements made from the hosts at the periphery. There have been a number of papers that estimate node and link parameters from end-to-end measurements from the hosts. Such parameters include link loss rates, delay distribution, and delay variances \cite{Bu2002,Duffield2002,presti2002multicast}, as well as traffic characteristics \cite{vardi1996network}. The use of multicast-based packets to derive the source tree topology of a given host has been well studied. The main idea is to send multicast packets from a source to multiple destinations and derive the source tree by correlating the delay or loss \cite{Duffield2002, presti2002multicast,caceres1999multicast}. If multicast is not available, there is prior literature on using a train of unicast packets instead \cite{Duffield2006}. Our techniques for collecting PSM metrics using a train of unicast packets on DETER is directly derived from prior work above that uses such techniques to construct the source trees. It has also pointed out in prior literature measuring PSMs from unicast probes can be error-prone \cite{Duffield2006}, which was also our observation in our DETER experiments. Going beyond inferring source trees, there is some literature on  merging multiple source trees to understand how the trees overlap within the network \cite{Coates2003,Rabbat2004}. There has also been recent work that derives conditions for a network to be reconstructible \cite{Berkolaiko2018}. However, our work is the first to provide a theoretical approach for inferring the complete network topology and routing paths and show that it works well for a wide range of real-world networks.}
\end{comment}



